Cross-modal Learning for Multi-modal Video Categorization

Multi-modal machine learning (ML) models can process data in multiple modalities (e.g., video, audio, text) and are useful for video content analysis in a variety of problems (e.g., object detection, scene understanding, activity recognition). In this paper, we focus on the problem of video categorization using a multi-modal ML technique. In particular, we have developed a novel multi-modal ML approach that we call "cross-modal learning", where one modality influences another but only when there is correlation between the modalities -- for that, we first train a correlation tower that guides the main multi-modal video categorization tower in the model. We show how this cross-modal principle can be applied to different types of models (e.g., RNN, Transformer, NetVLAD), and demonstrate through experiments how our proposed multi-modal video categorization models with cross-modal learning out-perform strong state-of-the-art baseline models.

==> sections/acknowledgements.tex <==
\section{Acknowledgements}
This work was supported in part by NSF, AFRL, DARPA, Siemens, Samsung, Google, Amazon, ONR YIPs and ONR Grants N00014-16-1-\{2713,2793\}. The views and conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of the U.S. Government, or any sponsor.

==> sections/dataset.tex <==
\section{Human Attention data}

In this section we provide more details about the data we use for HINT supervision. 
As mentioned in Section, we use the Human ATtention (HAT) \cite{human_attention} dataset by Das \etal for supervising VQA models using HINT. 
HAT maps are available for a total of 40554 image-question pairs.  
This corresponds to approximately 6 \% of the VQA dataset which consists of a total of 658111 image-question pairs (train + val). 
We used a total of 32256 HAT maps for training and 8192 maps for validation. 
%For the model trained on VQAv2 dataset we use maps for training and  maps for 

For image captioning we use the segmentation maps from the COCO \cite{LinECCV14coco} dataset as human attention. 
\cite{LinECCV14coco} provides segmentation annotations for 120K images corresponding to 80 everyday occurring objects. 

==> sections/hierarchical.tex <==
\section{Hierarchical Label Space}

TODO: Decide whether this will stay in the final paper version.


We have a hierarchical label in our domain, since we’re predicting tags in a hierarchical tag taxonomy. We would like to have a hierarchical loss function that will take this hierarchical structure of the label space into account while training the final layer. For example, let's consider that the actual label is {\em Action::War}. If we predict {\em Action::War} to be the most likely label, then the loss should be low. If we predict {\em Comedy}, then the loss should be high since the model predicted a different branch of the hierarchy. If, however, we predict {\em Action}, then the loss should have a medium value since the classifier matched the first part of the hierarchy (and hence should get some partial credit).

In order to define the hierarchical loss function $L_{classfn\_hier}$, we first consider the label space $K$ to be organized as a hierarchical tree, where every node in the tree corresponds to a class label. Let  $l(k)$ be the level corresponding to class $k$ in the hierarchy. 
%Other weightings such as $l$, $log l$ can %also be used. Alternatively,
In this case we consider $y_{i,j} = 1$ for all $j$ that is an ancestor of the actual class for $x_i$ in the hierarchy (except the root).
We define $g(y_i)$ as the lowest level of a class in $y_i$, defined as:
\begin{equation}
\label{eqn:gy}
g(y_i) = max(\{l(j): \forall j, y_{i,j}  = 1\}).
\end{equation}
Let us also define the following indicator function $I$:
\[
I(i, k) = \left\{
  \begin{array}{ll}
    1 & : \hat{y_i} = k \\
    0 & : \mbox{otherwise}
  \end{array}
\right.
\]
We can then define a function $f_{hier}(k, i)$ to give partial credit when the classifier predicts a node $k$ along the parent path of the actual node $y_i$ that is deeper in the taxonomy:
\begin{equation}
f_{hier}(i, k) = 2^{l(k) - g(y_i)}.I(i, k)
\end{equation}
We consider the multiclass variant of cross entropy loss. In the hierarchical case we scale
the loss by the partial credit weight $f_{hier}(k, i)$, giving us the following definition of hierarchical classification loss:

\begin{eqnarray}
L_{classfn\_hier} = -\frac{1}{N} \sum_{i=1}^N \sum_{k=1}^K f_{hier}(i, k) 
.(y_{i,k} \log \hat{y}_{i,k})
\end{eqnarray}

%Let us consider the general multiclass cross entropy loss, as introduced in Equation~\ref{eqn:classification_loss}. The indicator function $I$ in the equation is 1 when the predicted class is same as the actual class label, and 0 otherwise. In the hierarchical case, we have another option -- if we the predicted class is a parent of the actual class in the hierarchical tree, then we consider the prediction to be partially correct (with a correctness score determined by $f_{hier}(k, i)$). We define the hierarchical indicator function $H$ as:

%\[
%H(k, i) = \left\{
%  \begin{array}{ll}
%    1 & : \hat{y_i} = k \\
%    f_{hier}(k, i) & : k \in %\mbox{parents}(\hat{y_i}) \\
%    0 & : \mbox{otherwise}
%  \end{array}
%\right.
%\]
%where parents is a function that returns all the parents of any level in the hierarchy.
%Based on this definition, we now define the hierarchical classification loss as:

%\[
%L_{classification\_hier} = -\frac{1}{N} \sum_{i=1}^N \sum_{k=1}^K H(k,i) \log p( \hat{y_i} = k | x_i).
%\]

% Note that the hierarchical loss function can be instantiated in different ways, e.g., instead of 0.5 for the indicator value when the prediction is a parent of the actual value, we can use a value that depends on the length of the path between the ground truth and prediction values.

%One of the ideas we are considering in this space is using a variant of Huffman coding to design this hierarchical label loss function.

%We also want to consider a hierarchical attention model --- at the frame level we can have attention variables for the experts, while at the segment level we can have attention variables corresponding to a sequence of experts. This hierarchical attention model can help us attend to the relevant frames in the segment as well as to the relevant segments in the video.
